BSDP: Brain-inspired Streaming Dual-level Perturbations for Online Open World Object Detection

Humans can easily distinguish the known and unknown categories and can recognize the unknown object by learning it once instead of repeating it many times without forgetting the learned object. Hence, we aim to make deep learning models simulate the way people learn. We refer to such a learning manner as OnLine Open World Object Detection(OLOWOD). Existing OWOD approaches pay more attention to the identification of unknown categories, while the incremental learning part is also very important. Besides, some neuroscience research shows that specific noises allow the brain to form new connections and neural pathways which may improve learning speed and efficiency. In this paper, we take the dual-level information of old samples as perturbations on new samples to make the model good at learning new knowledge without forgetting the old knowledge. Therefore, we propose a simple plug-and-play method, called Brain-inspired Streaming Dual-level Perturbations(BSDP), to solve the OLOWOD problem. Specifically, (1) we first calculate the prototypes of previous categories and use the distance between samples and the prototypes as the sample selecting strategy to choose old samples for replay; (2) then take the prototypes as the streaming feature-level perturbations of new samples, so as to improve the plasticity of the model through revisiting the old knowledge; (3) and also use the distribution of the features of the old category samples to generate adversarial data in the form of streams as the data-level perturbations to enhance the robustness of the model to new categories. We empirically evaluate BSDP on PASCAL VOC and MS-COCO, and the excellent results demonstrate the promising performance of our proposed method and learning manner.

==> cas-refs.tex <==
\bibitem{DBLP:journals/ijcv/EveringhamGWWZ10}
M.~Everingham, L.~V. Gool, C.~K.~I. Williams, J.~M. Winn, and A.~Zisserman, ``The pascal visual object classes {(VOC)} challenge,'' \emph{Int. J. Comput. Vis.}, vol.~88, no.~2, pp. 303--338, 2010.

\bibitem{DBLP:conf/eccv/LinMBHPRDZ14}
T.~Lin, M.~Maire, S.~J. Belongie, J.~Hays, P.~Perona, D.~Ramanan, P.~Doll{\'{a}}r, and C.~L. Zitnick, ``Microsoft {COCO:} common objects in context,'' in \emph{Computer Vision - {ECCV} 2014 - 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part {V}}, ser. Lecture Notes in Computer Science, D.~J. Fleet, T.~Pajdla, B.~Schiele, and T.~Tuytelaars, Eds., vol. 8693.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2014, pp. 740--755.

\bibitem{mccloskey1989catastrophic}
M.~McCloskey and N.~J. Cohen, ``Catastrophic interference in connectionist networks: The sequential learning problem,'' in \emph{Psychology of learning and motivation}.\hskip 1em plus 0.5em minus 0.4em\relax Elsevier, 1989, vol.~24, pp. 109--165.

\bibitem{DBLP:conf/annes/Robins93a}
A.~V. Robins, ``Catastrophic forgetting in neural networks: the role of rehearsal mechanisms,'' in \emph{First New Zealand International Two-Stream Conference on Artificial Neural Networks and Expert Systems, {ANNES} '93, Dunedin, New Zealand, November 24-26, 1993}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 1993, pp. 65--68.

\bibitem{DBLP:conf/iccv/ShmelkovSA17}
K.~Shmelkov, C.~Schmid, and K.~Alahari, ``Incremental learning of object detectors without catastrophic forgetting,'' in \emph{{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice, Italy, October 22-29, 2017}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE} Computer Society, 2017, pp. 3420--3429.

\bibitem{DBLP:conf/cvpr/YoshihashiSKYIN19}
R.~Yoshihashi, W.~Shao, R.~Kawakami, S.~You, M.~Iida, and T.~Naemura, ``Classification-reconstruction learning for open-set recognition,'' in \emph{{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2019, Long Beach, CA, USA, June 16-20, 2019}.\hskip 1em plus 0.5em minus 0.4em\relax Computer Vision Foundation / {IEEE}, 2019, pp. 4016--4025.

\bibitem{DBLP:conf/wacv/DhamijaGVB20}
A.~R. Dhamija, M.~G{\"{u}}nther, J.~Ventura, and T.~E. Boult, ``The overlooked elephant of object detection: Open set,'' in \emph{{IEEE} Winter Conference on Applications of Computer Vision, {WACV} 2020, Snowmass Village, CO, USA, March 1-5, 2020}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2020, pp. 1010--1019.

\bibitem{DBLP:conf/cvpr/Joseph0KB21}
K.~J. Joseph, S.~H. Khan, F.~S. Khan, and V.~N. Balasubramanian, ``Towards open world object detection,'' in \emph{{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2021, virtual, June 19-25, 2021}.\hskip 1em plus 0.5em minus 0.4em\relax Computer Vision Foundation / {IEEE}, 2021, pp. 5830--5840.

\bibitem{DBLP:conf/icip/YuML0X22}
J.~Yu, L.~Ma, Z.~Li, Y.~Peng, and S.~Xie, ``Open-world object detection via discriminative class prototype learning,'' in \emph{2022 {IEEE} International Conference on Image Processing, {ICIP} 2022, Bordeaux, France, 16-19 October 2022}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2022, pp. 626--630.

\bibitem{DBLP:conf/cvpr/BendaleB15}
A.~Bendale and T.~E. Boult, ``Towards open world recognition,'' in \emph{{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2015, Boston, MA, USA, June 7-12, 2015}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE} Computer Society, 2015, pp. 1893--1902.

\bibitem{DBLP:journals/pami/RenHG017}
S.~Ren, K.~He, R.~B. Girshick, and J.~Sun, ``Faster {R-CNN:} towards real-time object detection with region proposal networks,'' \emph{{IEEE} Trans. Pattern Anal. Mach. Intell.}, vol.~39, no.~6, pp. 1137--1149, 2017.

\bibitem{DBLP:conf/eccv/LiH16}
Z.~Li and D.~Hoiem, ``Learning without forgetting,'' in \emph{Computer Vision - {ECCV} 2016 - 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part {IV}}, ser. Lecture Notes in Computer Science, B.~Leibe, J.~Matas, N.~Sebe, and M.~Welling, Eds., vol. 9908.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2016, pp. 614--629.

\bibitem{DBLP:conf/cvpr/RebuffiKSL17}
S.~Rebuffi, A.~Kolesnikov, G.~Sperl, and C.~H. Lampert, ``icarl: Incremental classifier and representation learning,'' in \emph{2017 {IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE} Computer Society, 2017, pp. 5533--5542.

\bibitem{DBLP:journals/prl/PengZL20}
C.~Peng, K.~Zhao, and B.~C. Lovell, ``Faster {ILOD:} incremental learning for object detectors based on faster {RCNN},'' \emph{Pattern Recognit. Lett.}, vol. 140, pp. 109--115, 2020.

\bibitem{DBLP:journals/pami/JosephRKKB22}
K.~J. Joseph, J.~Rajasegaran, S.~H. Khan, F.~S. Khan, and V.~N. Balasubramanian, ``Incremental object detection via meta-learning,'' \emph{{IEEE} Trans. Pattern Anal. Mach. Intell.}, vol.~44, no.~12, pp. 9209--9216, 2022.

\bibitem{DBLP:conf/icml/SerraSMK18}
J.~Serr{\`{a}}, D.~Suris, M.~Miron, and A.~Karatzoglou, ``Overcoming catastrophic forgetting with hard attention to the task,'' in \emph{Proceedings of the 35th International Conference on Machine Learning, {ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15, 2018}, ser. Proceedings of Machine Learning Research, J.~G. Dy and A.~Krause, Eds., vol.~80.\hskip 1em plus 0.5em minus 0.4em\relax {PMLR}, 2018, pp. 4555--4564.

\bibitem{DBLP:conf/cvpr/TiwariKIS22}
R.~Tiwari, K.~Killamsetty, R.~K. Iyer, and P.~Shenoy, ``{GCR:} gradient coreset based replay buffer selection for continual learning,'' in \emph{{IEEE/CVF} Conference on Computer Vision and Pattern Recognition, {CVPR} 2022, New Orleans, LA, USA, June 18-24, 2022}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2022, pp. 99--108.

\bibitem{DBLP:conf/nips/SunLS0W22}
Q.~Sun, F.~Lyu, F.~Shang, W.~Feng, and L.~Wan, ``Exploring example influence in continual learning,'' in \emph{Advances in Neural Information Processing Systems 35: Annual Conference on Neural Information Processing Systems 2022, NeurIPS 2022, New Orleans, LA, USA, November 28 - December 9, 2022}, S.~Koyejo, S.~Mohamed, A.~Agarwal, D.~Belgrave, K.~Cho, and A.~Oh, Eds., 2022, pp. 27\,075--27\,086.

\bibitem{DBLP:conf/cvpr/Gu0WD22}
Y.~Gu, X.~Yang, K.~Wei, and C.~Deng, ``Not just selection, but exploration: Online class-incremental continual learning via dual view consistency,'' in \emph{{IEEE/CVF} Conference on Computer Vision and Pattern Recognition, {CVPR} 2022, New Orleans, LA, USA, June 18-24, 2022}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2022, pp. 7432--7441.

\bibitem{Kirkpatrick_2017}
J.~Kirkpatrick, R.~Pascanu, N.~Rabinowitz, J.~Veness, G.~Desjardins, A.~A. Rusu, K.~Milan, J.~Quan, T.~Ramalho, A.~Grabska-Barwinska, D.~Hassabis, C.~Clopath, D.~Kumaran, and R.~Hadsell, ``Overcoming catastrophic forgetting in neural networks,'' \emph{Proceedings of the National Academy of Sciences}, vol. 114, no.~13, pp. 3521--3526, 2017.

\bibitem{DBLP:conf/eccv/AljundiBERT18}
R.~Aljundi, F.~Babiloni, M.~Elhoseiny, M.~Rohrbach, and T.~Tuytelaars, ``Memory aware synapses: Learning what (not) to forget,'' in \emph{Computer Vision - {ECCV} 2018 - 15th European Conference, Munich, Germany, September 8-14, 2018, Proceedings, Part {III}}, ser. Lecture Notes in Computer Science, vol. 11207.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2018, pp. 144--161.

\bibitem{DBLP:conf/cvpr/BendaleB16}
A.~Bendale and T.~E. Boult, ``Towards open set deep networks,'' in \emph{2016 {IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE} Computer Society, 2016, pp. 1563--1572.

\bibitem{DBLP:conf/eccv/BansalSSCD18}
A.~Bansal, K.~Sikka, G.~Sharma, R.~Chellappa, and A.~Divakaran, ``Zero-shot object detection,'' in \emph{Computer Vision - {ECCV} 2018 - 15th European Conference, Munich, Germany, September 8-14, 2018, Proceedings, Part {I}}, ser. Lecture Notes in Computer Science, V.~Ferrari, M.~Hebert, C.~Sminchisescu, and Y.~Weiss, Eds., vol. 11205.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2018, pp. 397--414.

\bibitem{DBLP:conf/icra/MillerNDS18}
D.~Miller, L.~Nicholson, F.~Dayoub, and N.~S{\"{u}}nderhauf, ``Dropout sampling for robust object detection in open-set conditions,'' in \emph{2018 {IEEE} International Conference on Robotics and Automation, {ICRA} 2018, Brisbane, Australia, May 21-25, 2018}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2018, pp. 1--7.

\bibitem{DBLP:conf/cvpr/HeZRS16}
K.~He, X.~Zhang, S.~Ren, and J.~Sun, ``Deep residual learning for image recognition,'' in \emph{2016 {IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE} Computer Society, 2016, pp. 770--778.

\bibitem{wu2019detectron2}
Y.~Wu, A.~Kirillov, F.~Massa, W.-Y. Lo, and R.~Girshick, ``Detectron2 github,'' \url{https://github.com/facebookresearch/detectron2}, 2019.

\bibitem{DBLP:conf/iclr/RiemerCALRTT19}
M.~Riemer, I.~Cases, R.~Ajemian, M.~Liu, I.~Rish, Y.~Tu, and G.~Tesauro, ``Learning to learn without forgetting by maximizing transfer and minimizing interference,'' in \emph{7th International Conference on Learning Representations, {ICLR} 2019, New Orleans, LA, USA, May 6-9, 2019}.\hskip 1em plus 0.5em minus 0.4em\relax OpenReview.net, 2019, pp. 1--31.

\bibitem{DBLP:conf/nips/ShinLKK17}
H.~Shin, J.~K. Lee, J.~Kim, and J.~Kim, ``Continual learning with deep generative replay,'' in \emph{Advances in Neural Information Processing Systems 30: Annual Conference on Neural Information Processing Systems 2017, December 4-9, 2017, Long Beach, CA, {USA}}, I.~Guyon, U.~von Luxburg, S.~Bengio, H.~M. Wallach, R.~Fergus, S.~V.~N. Vishwanathan, and R.~Garnett, Eds., 2017, pp. 2990--2999.

\bibitem{DBLP:journals/ijon/RamapuramGK20}
J.~Ramapuram, M.~Gregorova, and A.~Kalousis, ``Lifelong generative modeling,'' \emph{Neurocomputing}, vol. 404, pp. 381--400, 2020.

\bibitem{miller2019functions}
S.~M. Miller and A.~Sahay, ``Functions of adult-born neurons in hippocampal memory interference and indexing,'' \emph{Nature neuroscience}, vol.~22, no.~10, pp. 1565--1575, 2019.

\bibitem{van2022using}
O.~Van~der Groen, W.~Potok, N.~Wenderoth, G.~Edwards, J.~B. Mattingley, and D.~Edwards, ``Using noise for the better: The effects of transcranial random noise stimulation on the brain and behavior,'' \emph{Neuroscience \& Biobehavioral Reviews}, vol. 138, p. 104702, 2022.

\bibitem{mccormick1999spontaneous}
D.~A. McCormick, ``Spontaneous activity: signal or noise?'' \emph{Science}, vol. 285, no. 5427, pp. 541--543, 1999.

\bibitem{DBLP:conf/nips/WangX00CH22}
Z.~Wang, Q.~Xu, Z.~Yang, Y.~He, X.~Cao, and Q.~Huang, ``Openauc: Towards auc-oriented open-set recognition,'' in \emph{Advances in Neural Information Processing Systems 35: Annual Conference on Neural Information Processing Systems 2022, NeurIPS 2022, New Orleans, LA, USA, November 28 - December 9, 2022}, S.~Koyejo, S.~Mohamed, A.~Agarwal, D.~Belgrave, K.~Cho, and A.~Oh, Eds., 2022, pp. 25\,033--25\,045.

\bibitem{DBLP:conf/aaai/LuXLCN22}
J.~Lu, Y.~Xu, H.~Li, Z.~Cheng, and Y.~Niu, ``{PMAL:} open set recognition via robust prototype mining,'' in \emph{Thirty-Sixth {AAAI} Conference on Artificial Intelligence, {AAAI} 2022, Thirty-Fourth Conference on Innovative Applications of Artificial Intelligence, {IAAI} 2022, The Twelveth Symposium on Educational Advances in Artificial Intelligence, {EAAI} 2022 Virtual Event, February 22 - March 1, 2022}.\hskip 1em plus 0.5em minus 0.4em\relax {AAAI} Press, 2022, pp. 1872--1880.

\bibitem{DBLP:conf/iccv/KongR21}
S.~Kong and D.~Ramanan, ``Opengan: Open-set recognition via open data generation,'' in \emph{2021 {IEEE/CVF} International Conference on Computer Vision, {ICCV} 2021, Montreal, QC, Canada, October 10-17, 2021}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2021, pp. 793--802.

\bibitem{DBLP:conf/iccv/WangWSG21}
J.~Wang, X.~Wang, Y.~Shang{-}Guan, and A.~Gupta, ``Wanderlust: Online continual object detection in the real world,'' in \emph{2021 {IEEE/CVF} International Conference on Computer Vision, {ICCV} 2021, Montreal, QC, Canada, October 10-17, 2021}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2021, pp. 10\,809--10\,818.

\bibitem{Cokelaer2014}
T.~Cokelaer, ``Fitter github,'' \url{https://github.com/cokelaer/fitter}, 2014.

\bibitem{YANG2022108863}
D.~Yang, Y.~Zhou, A.~Zhang, X.~Sun, D.~Wu, W.~Wang, and Q.~Ye, ``Multi-view correlation distillation for incremental object detection,'' \emph{Pattern Recognition}, vol. 131, p. 108863, 2022.

\bibitem{ZHUANG2022108907}
C.~Zhuang, S.~Huang, G.~Cheng, and J.~Ning, ``Multi-criteria selection of rehearsal samples for continual learning,'' \emph{Pattern Recognition}, vol. 132, p. 108907, 2022.

\bibitem{MA2023109280}
C.~Ma, X.~Pan, Q.~Ye, F.~Tang, W.~Dong, and C.~Xu, ``Crossrectify: Leveraging disagreement for semi-supervised object detection,'' \emph{Pattern Recognition}, vol. 137, p. 109280, 2023.

\bibitem{GUO2024110329}
Y.~Guo, H.~Yu, S.~Xie, L.~Ma, X.~Cao, and X.~Luo, ``Dsca: A dual semantic correlation alignment method for domain adaptation object detection,'' \emph{Pattern Recognition}, vol. 150, p. 110329, 2024.

\bibitem{SUN2023109561}
W.~Sun, Q.~Li, J.~Zhang, D.~Wang, W.~Wang, and Y.~ao~Geng, ``Exemplar-free class incremental learning via discriminative and comparable parallel one-class classifiers,'' \emph{Pattern Recognition}, vol. 140, p. 109561, 2023.

\bibitem{DONG2023109488}
N.~Dong, Y.~Zhang, M.~Ding, and Y.~Bai, ``Class-incremental object detection,'' \emph{Pattern Recognition}, vol. 139, p. 109488, 2023.

